Efficient Cluster Selection for Personalized Federated Learning: A Multi-Armed Bandit Approach

Federated learning (FL) offers a decentralized training approach for machine learning models, prioritizing data privacy. However, the inherent heterogeneity in FL networks, arising from variations in data distribution, size, and device capabilities, poses challenges in user federation. Recognizing this, Personalized Federated Learning (PFL) emphasizes tailoring learning processes to individual data profiles. In this paper, we address the complexity of clustering users in PFL, especially in dynamic networks, by introducing a dynamic Upper Confidence Bound (dUCB) algorithm inspired by the multi-armed bandit (MAB) approach. The dUCB algorithm ensures that new users can effectively find the best cluster for their data distribution by balancing exploration and exploitation. The performance of our algorithm is evaluated in various cases, showing its effectiveness in handling dynamic federated learning scenarios.

==> ref.tex <==



@article{donahue2021optimality,
  title={Optimality and stability in federated learning: A game-theoretic approach},
  author={Donahue, Kate and Kleinberg, Jon},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={1287--1298},
  year={2021}
}

@inproceedings{li2022expert,
  title={Expert-Calibrated Learning for Online Optimization with Switching Costs},
  author={Li, Pengfei and Yang, Jianyi and Ren, Shaolei},
  booktitle={Abstract Proceedings of the 2022 ACM SIGMETRICS/IFIP PERFORMANCE Joint International Conference on Measurement and Modeling of Computer Systems},
  pages={85--86},
  year={2022}
}



@ARTICLE{9264742,
  author={Yang, Zhaohui and Chen, Mingzhe and Saad, Walid and Hong, Choong Seon and Shikh-Bahaei, Mohammad},
  journal={IEEE Transactions on Wireless Communications}, 
  title={Energy Efficient Federated Learning Over Wireless Communication Networks}, 
  year={2021},
  volume={20},
  number={3},
  pages={1935-1949},
  doi={10.1109/TWC.2020.3037554}}

  @inproceedings{zhou2022joint,
  title={Joint optimization of energy consumption and completion time in federated learning},
  author={Zhou, Xinyu and Zhao, Jun and Han, Huimei and Guet, Claude},
  booktitle={2022 IEEE 42nd International Conference on Distributed Computing Systems (ICDCS)},
  pages={1005--1017},
  year={2022},
  organization={IEEE}
}

@article{li2020lotteryfl,
  title={Lotteryfl: Personalized and communication-efficient federated learning with lottery ticket hypothesis on non-iid datasets},
  author={Li, Ang and Sun, Jingwei and Wang, Binghui and Duan, Lin and Li, Sicheng and Chen, Yiran and Li, Hai},
  journal={arXiv preprint arXiv:2008.03371},
  year={2020}
}

@article{t2020personalized,
  title={Personalized federated learning with moreau envelopes},
  author={T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={21394--21405},
  year={2020}
}

@article{yang2023personalized,
  title={Personalized federated learning on non-iid data via group-based meta-learning},
  author={Yang, Lei and Huang, Jiaming and Lin, Wanyu and Cao, Jiannong},
  journal={ACM Transactions on Knowledge Discovery from Data},
  volume={17},
  number={4},
  pages={1--20},
  year={2023},
  publisher={ACM New York, NY}
}

@article{sui2022find,
  title={Find Your Friends: Personalized Federated Learning with the Right Collaborators},
  author={Sui, Yi and Wen, Junfeng and Lau, Yenson and Ross, Brendan Leigh and Cresswell, Jesse C},
  journal={arXiv preprint arXiv:2210.06597},
  year={2022}
}

@inproceedings{luo2021cost,
  title={Cost-effective federated learning design},
  author={Luo, Bing and Li, Xiang and Wang, Shiqiang and Huang, Jianwei and Tassiulas, Leandros},
  booktitle={IEEE INFOCOM 2021-IEEE Conference on Computer Communications},
  pages={1--10},
  year={2021},
  organization={IEEE}
}

@article{deng2020adaptive,
  title={Adaptive personalized federated learning},
  author={Deng, Yuyang and Kamani, Mohammad Mahdi and Mahdavi, Mehrdad},
  journal={arXiv preprint arXiv:2003.13461},
  year={2020}
}

@inproceedings{huang2021personalized,
  title={Personalized cross-silo federated learning on non-iid data},
  author={Huang, Yutao and Chu, Lingyang and Zhou, Zirui and Wang, Lanjun and Liu, Jiangchuan and Pei, Jian and Zhang, Yong},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={9},
  pages={7865--7873},
  year={2021}
}

@inproceedings{azizi2022mix,
  title={MIX-MAB: Reinforcement learning-based resource allocation algorithm for LoRaWAN},
  author={Azizi, Farzad and Teymuri, Benyamin and Aslani, Rojin and Rasti, Mehdi and Tolvaneny, Jesse and Nardelli, Pedro HJ},
  booktitle={2022 IEEE 95th Vehicular Technology Conference:(VTC2022-Spring)},
  pages={1--6},
  year={2022},
  organization={IEEE}
}

@inproceedings{shi2021federated,
  title={Federated multi-armed bandits},
  author={Shi, Chengshuai and Shen, Cong},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={11},
  pages={9603--9611},
  year={2021}
}

@article{xia2020multi,
  title={Multi-armed bandit-based client scheduling for federated learning},
  author={Xia, Wenchao and Quek, Tony QS and Guo, Kun and Wen, Wanli and Yang, Howard H and Zhu, Hongbo},
  journal={IEEE Transactions on Wireless Communications},
  volume={19},
  number={11},
  pages={7108--7123},
  year={2020},
  publisher={IEEE}
}

@inproceedings{larsson2021automated,
  title={Automated Collaborator Selection for Federated Learning with Multi-armed Bandit Agents},
  author={Larsson, Hannes and Riaz, Hassam and Ickin, Selim},
  booktitle={Proceedings of the 4th FlexNets Workshop on Flexible Networks Artificial Intelligence Supported Network Flexibility and Agility},
  pages={44--49},
  year={2021}
}

@inproceedings{donahue2021model,
  title={Model-sharing games: Analyzing federated learning under voluntary participation},
  author={Donahue, Kate and Kleinberg, Jon},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={6},
  pages={5303--5311},
  year={2021}
}

@article{meidani2022mab,
  title={MAB-OS: Multi-Armed Bandits Metaheuristic Optimizer Selection},
  author={Meidani, Kazem and Mirjalili, Seyedali and Farimani, Amir Barati},
  journal={Applied Soft Computing},
  volume={128},
  pages={109452},
  year={2022},
  publisher={Elsevier}
}

@INPROCEEDINGS{9839030,
  author={Chen, Ziru and Zhang, Ran and Cai, Lin X. and Cheng, Yu and Liu, Yong},
  booktitle={ICC 2022 - IEEE International Conference on Communications}, 
  title={A Deep Reinforcement Learning based Approach for NOMA-based Random Access Network with Truncated Channel Inversion Power Control}, 
  year={2022},
  volume={},
  number={},
  pages={1835-1840},
  doi={10.1109/ICC45855.2022.9839030}}
  
@article{wu2023fedab,
  title={FedAB: Truthful Federated Learning with Auction-based Combinatorial Multi-Armed Bandit},
  author={Wu, Chenrui and Zhu, Yifei and Zhang, Rongyu and Chen, Yun and Wang, Fangxin and Cui, Shuguang},
  journal={IEEE Internet of Things Journal},
  year={2023},
  publisher={IEEE}
}


@inproceedings{donahue2021model,
  title={Model-sharing games: Analyzing federated learning under voluntary participation},
  author={Donahue, Kate and Kleinberg, Jon},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={6},
  pages={5303--5311},
  year={2021}
}


@inproceedings{al2021reducing,
  title={Reducing communication overhead of federated learning through clustering analysis},
  author={Al-Saedi, Ahmed A and Boeva, Veselka and Casalicchio, Emiliano},
  booktitle={2021 IEEE Symposium on Computers and Communications (ISCC)},
  pages={1--7},
  year={2021},
  organization={IEEE}
}

@inproceedings{briggs2020federated,
  title={Federated learning with hierarchical clustering of local updates to improve training on non-IID data},
  author={Briggs, Christopher and Fan, Zhong and Andras, Peter},
  booktitle={2020 International Joint Conference on Neural Networks (IJCNN)},
  pages={1--9},
  year={2020},
  organization={IEEE}
}
@inproceedings{al2023group,
  title={Group-personalized federated learning for human activity recognition through cluster eccentricity analysis},
  author={Al-Saedi, Ahmed A and Boeva, Veselka},
  booktitle={International Conference on Engineering Applications of Neural Networks},
  pages={505--519},
  year={2023},
  organization={Springer}
}

@inproceedings{gonccalves2015upper,
  title={Upper confidence bound (UCB) algorithms for adaptive operator selection in MOEA/D},
  author={Gon{\c{c}}alves, Richard A and Almeida, Carolina P and Pozo, Aurora},
  booktitle={Evolutionary Multi-Criterion Optimization: 8th International Conference, EMO 2015, Guimar{\~a}es, Portugal, March 29--April 1, 2015. Proceedings, Part I 8},
  pages={411--425},
  year={2015},
  organization={Springer}
}

@INPROCEEDINGS{9413628,
  author={Gupta, Samarth and Chaudhari, Shreyas and Mukherjee, Subhojyoti and Joshi, Gauri and Yağan, Osman},
  booktitle={ICASSP 2021 - 2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
  title={A Unified Approach to Translate Classical Bandit Algorithms to Structured Bandits}, 
  year={2021},
  volume={},
  number={},
  pages={3360-3364},
  doi={10.1109/ICASSP39728.2021.9413628}}

@article{ghosh2020efficient,
  title={An efficient framework for clustered federated learning},
  author={Ghosh, Avishek and Chung, Jichan and Yin, Dong and Ramchandran, Kannan},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={19586--19597},
  year={2020}
}

@article{tan2022towards,
  title={Towards personalized federated learning},
  author={Tan, Alysa Ziying and Yu, Han and Cui, Lizhen and Yang, Qiang},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}

@article{tang2021personalized,
  title={Personalized federated learning with clustered generalization},
  author={Tang, Xueyang and Guo, Song and Guo, Jingcai},
  year={2021}
}

@article{marfoq2021federated,
  title={Federated multi-task learning under a mixture of distributions},
  author={Marfoq, Othmane and Neglia, Giovanni and Bellet, Aur{\'e}lien and Kameni, Laetitia and Vidal, Richard},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={15434--15447},
  year={2021}
}
